Holistic Robust Data-Driven Decisions

The design of data-driven formulations for machine learning and decision-making with good out-of-sample performance is a key challenge. The observation that good in-sample performance does not guarantee good out-of-sample performance is generally known as overfitting. Practical overfitting can typically not be attributed to a single cause but is caused by several factors simultaneously. We consider here three overfitting sources: (i) statistical error as a result of working with finite sample data, (ii) data noise, which occurs when the data points are measured only with finite precision, and finally, (iii) data misspecification in which a small fraction of all data may be wholly corrupted. Although existing data-driven formulations may be robust against one of these three sources in isolation, they do not provide holistic protection against all overfitting sources simultaneously. We design a novel data-driven formulation that guarantees such holistic protection and is computationally viable. Our distributionally robust optimization formulation can be interpreted as a novel combination of a Kullback-Leibler and L\'evy-Prokhorov robust optimization formulation. In the context of classification and regression problems, we show that several popular regularized and robust formulations naturally reduce to a particular case of our proposed novel formulation. Finally, we apply the proposed HR formulation to two real-life applications and study it alongside several benchmarks: (1) training neural networks on healthcare data, where we analyze various robustness and generalization properties in the presence of noise, labeling errors, and scarce data, (2) a portfolio selection problem with real stock data, and analyze the risk/return tradeoff under the natural severe distribution shift of the application.

==> figures/performance_plots/cvar-scatter.tex <==
\pgfplotsset{
  xticklabel style={/pgf/number format/fixed},
  yticklabel style={/pgf/number format/fixed}
}

\begin{tikzpicture}
  \begin{axis}[enlargelimits=false,
    clip=true,
    xlabel={-CVaR},
    ylabel={Expected Return},
    legend pos=north west,
    ymax = 0.1,
    % xticks = {-0.2, -0.15, -0.1, -0.05, 0, 0.05},
    xmax = 0.02,
    y label style={at={(-0.1,0.5)}},
    legend to name=named,
    legend style={legend cell align=left,align=left,draw=white!15!black,legend columns=3}
    ]

    \addplot+ [forget plot,
    only marks,
    mark=star,
    mark options={scale=0.4, purple!50},
    ] table[x=risk, y=return, col sep=comma] {figures/performance_plots/Markowitz_-cvar_perto-False.csv};
    
    \addplot+ [forget plot,
    only marks,
    mark=diamond*,
    mark options={scale=0.4, green!50},
    ] table[x=risk, y=return, col sep=comma] {figures/performance_plots/CVaR_-cvar_perto-False.csv};
    
    \addplot+ [forget plot,
    only marks,
    mark=square*,
    mark options={scale=0.4, red!50},
    ] table[x=risk, y=return, col sep=comma] {figures/performance_plots/W_-cvar_perto-False.csv};

    \addplot+ [forget plot,
    only marks,
    mark=triangle*,
    mark options={scale=0.4, orange!50},
    ] table[x=risk, y=return, col sep=comma] {figures/performance_plots/KL_-cvar_perto-False.csv};

    \addplot+ [forget plot,
    only marks,
    mark=*,
    mark options={scale=0.4, blue!50},
    ] table[x=risk, y=return, col sep=comma] {figures/performance_plots/HR_-cvar_perto-False.csv};

    %%% 

    \addplot+ [
    only marks,
    mark=star,
    mark options={scale=1, purple},
    ] table[x=risk, y=return, col sep=comma] {figures/performance_plots/Markowitz_-cvar_perto-True.csv};
    \addlegendentry{Markowitz}
    
    \addplot+ [
    only marks,
    mark=diamond*,
    mark options={scale=1, green},
    ] table[x=risk, y=return, col sep=comma] {figures/performance_plots/CVaR_-cvar_perto-True.csv};
    \addlegendentry{CVaR}

    \addplot+ [
    only marks,
    mark=square*,
    mark options={scale=0.8, red},
    ] table[x=risk, y=return, col sep=comma] {figures/performance_plots/W_-cvar_perto-True.csv};
    \addlegendentry{Wasserstein}


    \addplot+ [
    only marks,
    mark=triangle*,
    mark options={scale=0.8, orange},
    ] table[x=risk, y=return, col sep=comma] {figures/performance_plots/KL_-cvar_perto-True.csv};
    \addlegendentry{Kullbacl-Leibler}

    \addplot+ [
    only marks,
    mark=*,
    mark options={scale=0.8, blue},
    ] table[x=risk, y=return, col sep=comma] {figures/performance_plots/HR_-cvar_perto-True.csv};
    \addlegendentry{Holistic Robust}

  \end{axis}
\end{tikzpicture}

==> figures/performance_plots/std-scatter.tex <==
\pgfplotsset{
  xticklabel style={/pgf/number format/fixed},
  yticklabel style={/pgf/number format/fixed}
}

\begin{tikzpicture}
  \begin{axis}[enlargelimits=false,
    clip=true,
    xlabel={Standard Deviation},
    ylabel={Expected Return},
    legend pos=south west,
    ymax = 0.1,
    % xticks = {-0.2, -0.15, -0.1, -0.05, 0, 0.05},
    % xmax = 0.05,
    y label style={at={(-0.1,0.5)}},
    legend to name=named,
    legend style={legend cell align=left,align=left,draw=white!15!black,legend columns=3}
    ]

    \addplot+ [forget plot,
    only marks,
    mark=star,
    mark options={scale=0.4, purple!50},
    ] table[x=risk, y=return, col sep=comma] {figures/performance_plots/Markowitz_std_perto-False.csv};

    \addplot+ [forget plot,
    only marks,
    mark=diamond*,
    mark options={scale=0.4, green!50},
    ] table[x=risk, y=return, col sep=comma] {figures/performance_plots/CVaR_std_perto-False.csv};
    
    \addplot+ [forget plot,
    only marks,
    mark=square*,
    mark options={scale=0.4, red!50},
    ] table[x=risk, y=return, col sep=comma] {figures/performance_plots/W_std_perto-False.csv};

    \addplot+ [forget plot,
    only marks,
    mark=triangle*,
    mark options={scale=0.4, orange!50},
    ] table[x=risk, y=return, col sep=comma] {figures/performance_plots/KL_std_perto-False.csv};

    \addplot+ [forget plot,
    only marks,
    mark=*,
    mark options={scale=0.4, blue!50},
    ] table[x=risk, y=return, col sep=comma] {figures/performance_plots/HR_std_perto-False.csv};

    %%% 

    \addplot+ [
    only marks,
    mark=star,
    mark options={scale=1, purple},
    ] table[x=risk, y=return, col sep=comma] {figures/performance_plots/Markowitz_std_perto-True.csv};
    \addlegendentry{Markowitz}
    
    \addplot+ [
    only marks,
    mark=diamond*,
    mark options={scale=1, green},
    ] table[x=risk, y=return, col sep=comma] {figures/performance_plots/CVaR_std_perto-True.csv};
    \addlegendentry{CVaR}

    \addplot+ [
    only marks,
    mark=square*,
    mark options={scale=0.8, red},
    ] table[x=risk, y=return, col sep=comma] {figures/performance_plots/W_std_perto-True.csv};
    \addlegendentry{Wasserstein}


    \addplot+ [
    only marks,
    mark=triangle*,
    mark options={scale=0.8, orange},
    ] table[x=risk, y=return, col sep=comma] {figures/performance_plots/KL_std_perto-True.csv};
    \addlegendentry{Kullback-Leibler}

    \addplot+ [
    only marks,
    mark=*,
    mark options={scale=0.8, blue},
    ] table[x=risk, y=return, col sep=comma] {figures/performance_plots/HR_std_perto-True.csv};
    \addlegendentry{Holistic Robust}

  \end{axis}
\end{tikzpicture}
